Fairness in ERC token markets: A Case Study of CryptoKitties

Fairness is an important trait of open, free markets. Ethereum is a platform meant to enable digital, decentralized markets. Though many researchers debate the market's fairness, there are few discussions around the fairness of automated markets, such as those hosted on Ethereum. In this paper, using pilot studies, we consider unfair factors caused by adding the program. Because CryptoKitties is one of the major blockchain-based games and has been in operation for an extended period of time, we focus on its market to examine fairness. As a result, we concluded that a gene determination algorithm in this game has little randomness, and a significant advantage to gain profit is given to players who know its bias over those who do not. We state incompleteness and impact of the algorithm and other factors. Besides, we suppose countermeasures to reduce CryptoKitties' unfairness as a market.

==> 002_background.tex <==
\section{Background}
In this section, we describe blockchain, Smart Contract, and CryptoKitties.
\subsection{Blockchain}
\paragraph{} Blockchain is a cryptocurrency ledger. Satoshi Nakamoto proposed it as a bitcoin ledger in 2010. It consists of many blocks. Each block contains transactions, a timestamp, a previous hash, and a nonce. A transaction has a sender address, a recipient address, value, and timestamp. These addresses have anonymity so that people can't figure out a real person who has the address. A previous hash is the previous block's hash. The block information is succeed as a hash value. If a transaction is changed, its block hash value will be also changed, and we can see it was dishonest. Thus, blockchain has anti-tamperability. A block creator chooses the block that he thinks all transaction in it are honest. This block hash value will be the previous hash. Transactions in the block that has six child blocks are legimated. A nonce is used when a new block is created. This block's hash value is too small so that it takes some time to make the block. Creating a new block means that a ledger is updated. If it takes less time, many people can create blocks, and a lot of transactions that may includes dishonest ones will be uploaded on blockchain. In order to avoid this situation, we need "nonce."  However, all participants can create block if someone find the nonce so that its block hash value is less than threshold. So, there is no administer. In blockchain, because everyone is equal and no administer exists, they can see all blocks. Therefore, blockchain is satisfied with a ledger requirements.

\subsection{Smart Contract}
\paragraph{} Nick Szabo proposed Smart Contract in 1994. We define a contract in advance. Everybody can not change it once defined. When a person agrees with its definition, the contract is executed. He and the contractor's settlement will be ran automatically. We need no third party to run this contract. Take a vender machine for example, the pre-definition is the price and picture of the product displayed. By selecting a juice, it is correctly executed until settlement.
\paragraph{} Ethereum has implemented Smart Contract for the first time. With writing pre-definition on blockchain, all users don't re-write it. After pre-definition, programming code Solidity runs contracts. Thanks to this system, we can exchange Ethereum safely.

\subsection{CryptoKitties}
\paragraph{} CryptoKitties is the most famous blockchain-based game. Axiom Zen made this game in 2017. Users are getting increasing year by year. Its number is more than one hundred thousand, and its economic effect is more than forty million dollars. 
In this game, users exchange Ethereum and ERC-721 tokens. ERC-721 is non-fungible token(NFT). Unlike cryptocurrency, NFTs are unique tokens, each with its parameters. Each ERC-721 token differs from its value. By birthing and trading ERC-721 tokens, users aim to earn Ethereum. This game's source code is written in Solidity. So, all trades in this game are executed by Smart Contract. Not only these trade data but ERC-721 token data are on blockchain.
\paragraph{} In CryptoKitties, an ERC-721 token is a kitty. Again, players exchange kitties and Ethereum. Users take part in a dutch auction that the exhibited kitty's price goes down as time passes so that they get a kitty. If a player wants to earn Ethereum, he can put his kitty up for auction. Besides, a kitty, you have can be a parent. A player selects two kitties. Or, he selects one kitty and rent one kitty. These two kitties will be parents. In the case of rental, he should participate in a birth parent auction. Its style is also dutch. After a breeding period that varies from kitty to kitty, a child kitty is born. These kitties have an ID, gene, and generation. A gene differs from each kitty, and it determines its appearance. A child kitty inherits its parents' gene, but sometimes happen mutation. It depends on the gene determination algorithm defined by Smart Contract. A child kitty's generation is the greater of the parents' generation plus one. Kitty's root, generation 0 kitties, are created by CryptoKitties creators, and the number of them is limited to 50,000. It was released every 15 minutes, and it was done handing them out in 2018.
\paragraph{} There are about 2 million kitties; the most enormous ID kitty is about 2 million. On a blockchain, there are each kitty's data in addition to transactions. We can analyze them using Etherscan that is a blockchain analysis website. Also, since CryptoKitties is a Smart Contract game, its source code is published. By using them, we research CryptoKitties' algorithm and its result.

==> 003_related_work.tex <==
\section{Related Work}
\paragraph{Alesja Serada et al.} He demonstrates the limits of scarcity in the value construction of CryptoKitties token owners. He uses open blockchain analytics and player-generated analytics created after one year of participant observation of the game as research materials. He asserts that unlike bitcoin, the number of kitties is no limit because a kitty can breed as many times as its owners want. It led to a decrease in its scarcity. Also, interestingly, despite generation 0 kitties are only 50,000, its price is getting decreasing. He says that there are other factors that kitty's value is down. One reason is the gas fee. Gas discourages new players join, and players continue to play for a long time because a high-cost transaction is executed on a priority basis. Because of it, CryptoKitties is not a zero-sum game. This fact contradicts that this game helps to increase kitty value. Also, he says that family Jewels, the stone symbols are given to cats that were introduced as inheritable rewards for kitties and are rare and sold quite a bit on the market by some players. Our research reveals its reason.

\paragraph{Charlotte et al.} He doubts that even though blockchain is said to replace the law, participants trade each other without trust that the law acknowledges. He argues that it is doubtful whether Dapps are really distributed applications because it has no proof. He focuses on some Dapps, including CryptoKitties. In the case of CryptoKitties, since it's possible that CryptoKitties is not decentralized, it may be misleading to users. The reason why kitty is considered immutable and cannot be taken away from others is the steadfast and tamper-proof properties of the blockchain. However, only the market uses its properties. Charlotte points out that it is a vulnerability, and some can cheat others to execute a dishonest contract. 
